Comparing Representations in Tracking for Event Camera-based SLAM

This paper investigates two typical image-type representations for event camera-based tracking: time surface (TS) and event map (EM). Based on the original TS-based tracker, we make use of these two representations' complementary strengths to develop an enhanced version. The proposed tracker consists of a general strategy to evaluate the optimization problem's degeneracy online and then switch proper representations. Both TS and EM are motion- and scene-dependent, and thus it is important to figure out their limitations in tracking. We develop six tracker variations and conduct a thorough comparison of them on sequences covering various scenarios and motion complexities. We release our implementations and detailed results to benefit the research community on event cameras: https: //github.com/gogojjh/ESVO_extension.

==> acknowled.tex <==
\ack
This work was supported by Collaborative Research Fund by Research Grants Council Hong Kong, 
under Project No. C4063-18G, Department of Science and Technology of Guangdong Province Fund, under Project No. GDST20EG54 and Zhongshan Municipal Science and Technology Bureau Fund, under project ZSST21EG06, awarded to Prof. Ming Liu.

==> computation_time.tex <==
\subsection{Computation Time}
\label{sec:exp_computation_time}

The average computational time of tracker variations is reported in Table \ref{tab:latency}, 
where all of them take around $7$-$8ms$ to solve the pose estimation problem.
Depending on the sensor resolution, the creation of the TS takes about $5$-$10ms$ \cite{zhou2020event}.
The degeneracy evaluation takes about $0.5$-$1.5ms$.

% \begin{table}[t]
%     \begin{center}
%         \renewcommand\arraystretch{1.0}
%         \renewcommand\tabcolsep{15pt}
%         \begin{tabular}{cc}
%             \toprule[0.03cm]
%             Tracker & Time [$ms$] \\
%             \toprule[0.03cm]
%             TS & $8.0\pm5.3$ \\
%             $\text{EM}_{2000}$ & $7.7\pm5.5$ \\
%             $\text{EM}_{3000}$ & $7.4\pm4.4$ \\
%             $\text{EM}_{4000}$ & $7.2\pm3.8$ \\
%             $\text{EM}_{5000}$ & $7.4\pm4.4$ \\
%             TS+$\text{EM}_{4000}$ &$6.6\pm3.0$ \\
%             \toprule[0.03cm]
%         \end{tabular}
%     \end{center}
%     \caption{Average latency [$ms$] of pose optimization in tracking.}
%     \label{tab:latency}
% \end{table}

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.98\linewidth]{figure/latency_time_change-crop.pdf}
%     \caption{xxx.}
%     \label{fig:latency_time_change}
% \end{figure}








==> discussion.tex <==
\subsection{Discussion}
\label{sec:exp_discussion}

The presented trackers have limitations. 
First, although the enhance TSEM-based tracker can mitigate the undesirable effect caused by the unreliable TS,
it suffers shortcommings of both the TS and EM if $\lambda_{th}$ is not well tuned.
This explains why the TSEM has bad accuracy on $\textit{simu\_poster\_6DoF}$, $\textit{simu\_checkerboard\_6DoF}$, and $\textit{rpg\_box}$.
Hence, the utilization of the TSEM is subtle: tunning a good parameter requies to know more about dataset, 
while the degeneracy check is used to evaluate the conditions in unfamiliar environments.

Second, we find that the estimated trajectories of the current tracker are not smooth. 
TS-based tracker's trajectory on $\textit{rpg\_monitor}$ is visualized in Fig. \ref{fig:TS_traj_rpg_monitor}.
This is due to the fact that the tracker lacks a regularization term in optimization.
Possible solutions can be introducing the motion prior \cite{forster2016svo} or considering historical measurements (sliding window-based framework \cite{qin2018vins} or full batch optimization \cite{mueggler2015continuous}).
Moreover, as done in monocular event camera with an IMU \cite{zihao2017event,rebecq2017real,vidal2018ultimate}, 
stereo event-based VIO is an unexplored but promissing direction for this problem.

Finally, the image-type representations quantize event timestamps. The tracking results can be further optimized by introducing spline-based optimization framework \cite{mueggler2018continuous,gentil2020idol}.

% 1. summarize the failures of TSs and EMs. Results are motion- and scene-dependent.

% 2. no perfect representation -> the pose estimates using only one event frame may fail; 
% also lack local consistency; 

% solution: 
% introduce motion-prior for regularization \cite{}, 
% use recent historical measurements (sliding window-based framework or full batch optimization (but offline)), 
% fuse with high-frequency sensor (i.e., IMUs) \cite{}


==> experiment__DESKTOP-GGU3OSC_s_conflicted_copy_2021-03-15_.tex <==
\section{Experimental Results}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tracking Evaluation}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Full System Evaluation}


\subsubsection{Simulated Experiment}



\subsubsection{Indoor Experiment}



\subsubsection{Outdoor Experiment}

==> experiment__ramlab-Alienware-15-R4_s_conflicted_copy_2021-03-21_.tex <==
\section{Experimental Results}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tracking Evaluation}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Full System Evaluation}


\subsubsection{Simulated Experiment}



\subsubsection{Indoor Experiment}



\subsubsection{Outdoor Experiment}

==> guideline.tex <==
\begin{abstract}
   The ABSTRACT is to be in fully-justified italicized text, at the top
   of the left-hand column, below the author and affiliation
   information. Use the word ``Abstract'' as the title, in 12-point
   Times, boldface type, centered relative to the column, initially
   capitalized. The abstract is to be in 10-point, single-spaced type.
   Leave two blank lines after the Abstract, then begin the main text.
   Look at previous CVPR abstracts to get a feel for style and length.
\end{abstract}

Please follow the steps outlined below when submitting your manuscript to
the IEEE Computer Society Press.  This style guide now has several
important modifications (for example, you are no longer warned against the
use of sticky tape to attach your artwork to the paper), so all authors
should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confYear~web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section,
must be no longer than eight pages in length. The references section
will not be included in the page count, and there is no limit on the
length of the references section. For example, a paper of eight pages
with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confYear.}

Overlength papers will simply not be reviewed.  This includes papers
where the margins and formatting are deemed to have been significantly
altered from those laid down by this style guide.  Note that this
\LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for
supervised revisions of manuscripts.  The reviewing process cannot determine
the suitability of the paper for presentation in eight pages if it is
reviewed in eleven.  

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document using a non-\LaTeX\
document preparation system, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. 
(\LaTeX\ users may use options of cvpr.cls to switch between different 
versions.)  
Reviewers:
note that the ruler measurements do not align well with lines in the paper
--- this turns out to be very difficult to do well when the paper contains
many figures and equations, and, when done, looks ugly.  Just use fractional
references (e.g.\ this line is $095.5$), although in most cases one would
expect that the approximate location will be adequate.

\subsection{Mathematics}

Please number all of your sections and displayed equations.  It is
important for readers to be able to refer to any particular equation.  Just
because you didn't refer to it in the text doesn't mean some future reader
might not need to refer to it.  It is cumbersome to have to use
circumlocutions like ``the equation second from the top of page 3 column
1''.  (Note that the ruler will not be present in the final copy, so is not
an alternative to equation numbers).  All authors will benefit from reading
Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.


\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind
review.  Blind review does not mean that one must remove
citations to one's own work---in fact it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  That is all.  (But see below for
techreports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith; it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith \etal [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time,
which covers similar or overlapping material, you may need to refer to that
submission in order to explain the differences, just as you would if you
had previously published related work.  In such cases, include the
anonymized parallel submission~\cite{Authors14} as additional material and
cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324,
Supplied as additional material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be
found elsewhere, and refer them to a technical report.  For conference
submissions, the paper must stand on its own, and not {\em require} the
reviewer to go to a techreport for further details.  Thus, you may say in
the body of the paper ``further details may be found
in~\cite{Authors14b}''.  Then submit the techreport as additional material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the CVPR70 audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention,
reads better than the first version, and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double blind review policy, you can report results of other challenge participants together with your results in your paper. For your results, however, you should not identify yourself and should not mention your participation in the challenge. Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``
   Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
\cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.
%
Page numbers should be in footer with page numbers, centered and .75
inches from the bottom of the page and make it start at the correct page
number rather than the 4321 in the example.  To do this fine the line (around
line 20)
\begin{verbatim}
\setcounter{page}{4321}
\end{verbatim}
where the number 4321 is your assigned starting page.



%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors14}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths which render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confYear~web page for a discussion
of the use of color in your document.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.

Please direct any questions to the production editor in charge of these
proceedings at the IEEE Computer Society Press: 
\url{https://www.computer.org/about/contact}.


{\small
\bibliographystyle{ieee_fullname}
\bibliography{egbib}
}

==> methodology__DESKTOP-GGU3OSC_s_conflicted_copy_2021-03-15_.tex <==
\section{Methodology}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{System Overview}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Event Representation}

\subsubsection{Pure Events}

\subsubsection{Negative Time Surface}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tracking}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mapping}

==> methodology__ramlab-Alienware-15-R4_s_conflicted_copy_2021-03-21_.tex <==
\section{Methodology}

\subsection{Formulation}
Given map and event representation, compute the 6-DoF transformations.

\subsection{Edge Map}


\subsection{Time Surface Map}



% \section{Methodology}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{System Overview}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% \subsection{Event Representation}
% \subsubsection{Pure Events}
% \subsubsection{Negative Time Surface}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Tracking}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Mapping}

==> note.tex <==
\section{Note}

\textbf{Issues of ESVO:}
\begin{enumerate}
    \item Local consistent, but globally inconsistent: Because tracking: ESVO utilizes the local map ($<40$ frames) or fixed number of point cloud; 
    mapping: fuse the near stereo observations
    \item Synchronous Time Surface: may degenerate if lacking events
\end{enumerate}

\textbf{Issues of EVO:}
\begin{enumerate}
    \item Local consistent, but globally inconsistent. Because tracking: EVO utilizes the local map (\ie, within the FOV) or fixed number of point cloud.
    \item Scale ambiguity
\end{enumerate}


==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Scholary works on event cameras are extensive. 
A more complete survey is provided in \cite{gallego2020event}.
Here we briefly review the most relevant works regrading this topic: event representations for camera tracking.

Depending on how many events are processed simultaneously, related algorithms can categorized as:
\textit{1)} methods that operate on an \textit{event-by-event bias} where the unknown state of the camera changes upon the arrival of a single event;
\textit{2)} methods that operate on \textit{packets or groups of events}.
The former can achieve the minimum latency, but commmonly carry few information and is subject to noise.
Filters, such as the Extended Kalman filter, are the dominant framework of these methods \cite{}.
In spite of introducing some latency, the latter 



Traditional paradigm presented in feature- or photometric-based trackers \cite{} are not feasible to this case 
since events are 



Unlike traditional cameras, event cameras 

event cameras represent a paradigm shift since visual information is: (i)
which is fundamentally different from a sequence of images. 
Such a paradigm shift calls for new methods to process visual in- formation and unlock the capabilities of these novel sensors.



frame cameras, event cameras acquire events in an asynchronous and sparse way.
Depending on how 




Related algorithms 

faciliate the data assocation between the model and events




Event are processed and often converted into various representations for track, 
which faciliate




The key problem of tracking is the data association between the model and events.



Instead of processing the individual event, 


xx is a xxx
played the crucial role in the front end of many event vision to facilitate subsequent tasks.

% Events are processed and often transformed into alternative representations (Fig. 3) 
% that facilitate the extraction of meaningful information (“features”) to solve a given task. 
% Here we review popular representations of event data. Several of them arise from the need to aggregate the little information
% conveyed by individual events in the absence of additional knowledge. Some representations are simple, hand-crafted
% data transformations whereas others are more elaborate.

% Hence, the temporal aspect, specially latency, plays an essential role in the way events are processed.
% Hence, the distinction between both categories is more subtle: an event alone does not provide enough information for estimation,
%   and so additional information, in the form of past events or extra knowledge, is needed. 

% extract meaningful information from the event dta to fulfill a given task.
% This is a very broad question, since the answer is application dependent, and it drives the algorithmic design of the task solver.

% Unlike pixels in traditional cameras, events are acquired in an asynchronous and sparse way with high temporal resolution.
% Depending on how many events are processed simultaneously, related algorithms are categorized into \textit{event-by-event} 
% and \textit{groups or packets of events} methods.

% overview of representations; the characteristics of representations of event-by-event and groups or packets of events
% Research on event-based camera localization has progressed by addressing scenarios of increasing complexity.

% Unlike traditional cameras, event cameras acquire information in an asynchronous and sparse way with high temporal resolution.
% To facilitate the extraction of features, events are often converted into various representations.

% ilters, such as
% the Extended Kalman filter, are the dominant framework of
% the event-by-event–based type of methods. I






==> tracking_evaluation.tex <==
\subsection{Tracking Evaluation}
\label{sec:tracking_evaluation}

We implement six tracker variations according to the used representations.
They are denoted by ``TS'', ``$\text{EM}_{2000}$'', ``$\text{EM}_{3000}$'', ``$\text{EM}_{4000}$'', ``$\text{EM}_{5000}$'', and ``TS+$\text{EM}_{4000}$'' respectively.
The subscript of ``EM'' indicates the number of events to generate an EM. 
``TS+$\text{EM}_{4000}$'' is the proposed tracker with the degeneracy check.
To evaluate their performance, we compute the pose accuracy using the absolute trajectory error (ATE) in translation \cite{zhang2018tutorial} w.r.t. the ground truth.
We conduct $10$-trial SLAM tests on each sequence.
The mean ATE is reported in Table \ref{tab:ATE}.

All trackers achieve similar accuracy on the simplest sequences (\textit{simu\_X\_planar}), 
while their results show worse accuracy on more complex sequences.
We cannot directly determine the ``best'' representations according to the accuracies since all trackers may have large errors on some sequences.
We should analyze the results by considering the characteristics of scenes and motion.
The TS-based tracker outperform others on \textit{simu\_office\_6DoF}, \textit{rpg\_bin}, and \textit{rpg\_box},
where high-contrast textures (e.g., lines) are presented (see Fig. \ref{fig:scene_image}). 
For EM-based trackers, we observe that their optimization fails on these sequences and thus results in low accuracy.
Fig. \ref{fig:EM_tracking_fail} illustrates three failure cases.

\begin{table}[t]
    \begin{center}
        \renewcommand\arraystretch{1.0}
        \renewcommand\tabcolsep{3pt}
        \begin{tabular}{cccccc}
            \toprule[0.03cm]
            TS & $\text{EM}_{2000}$ & $\text{EM}_{3000}$ & $\text{EM}_{4000}$ & $\text{EM}_{5000}$ & TS+$\text{EM}_{4000}$\\
            \toprule[0.03cm]
            $8\pm5$ & $8\pm6$ & $7\pm4$ & $7\pm4$ & $7\pm4$& $7\pm3$ \\
            \toprule[0.03cm]
        \end{tabular}
    \end{center}
    \caption{Average computation time [$ms$] of trackers.}
    \label{tab:latency}
\end{table}

\begin{figure}[t]
    \centering\includegraphics[width=0.995\linewidth]{figure/traj_rpg_monitor-crop.pdf}
    \caption{TS's trajectory on $\textit{rpg\_monitor}$.}
    \label{fig:TS_traj_rpg_monitor}
\end{figure}

On the other hand, EM-based trackers consistently have better performance than the TS-based counterpart on \textit{upenn\_indoor\_flying3}.
We note that few events are generated in this sequence, and thus the TS triggered at a constant rate becomes unreliable when the drone stops and hovers.
Not enough constraints make the optimization degenerate or fail.
An example is shown in Fig. \ref{fig:tracking_deg}, 
with the plot displaying the value of the \textit{degeneracy factor} $\lambda$ on sequences: \textit{simu\_office\_6DoF}, \textit{rpg\_box}, and \textit{upenn\_indoor\_flying3}.
Regarding \textit{upenn\_indoor\_flying3}, at the time of $8.2s$, the TS-based tracker degenerates due to the unreliable TS (see Fig. \ref{fig:tracking_deg_reproj_ts}).
The corresponding \textit{factor} $\lambda$ is smaller than the threshold.
Therefore, we can swith the stable EM and then redo the tracking, improving the tracker's results.

The trajectories produced by the TS-based tracker on all sequences are compared 
in Fig. \ref{fig:simu_dof_plot}, Fig. \ref{fig:rpg_dof_plot}, and Fig. \ref{fig:upenn_dof_plot}.
Due to limited space, only the ground truth trajectories and trajectories of the tracker with the highest accuracy are shown as the reference.
Through these figures, readers can have a better understanding of the above explanations.
For example, we observe that the poses of the TS-based tracker "jump" on \textit{upenn\_indoor\_flying3} from Fig. \ref{fig:upenn_dof_plot}.
The unreliable TS causes degrades this performance.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subfigure[\textit{simu\_poster}]
% {
%     \hfill\centering\includegraphics[width=0.33\linewidth]{figure/scene/scene_simu_poster.png}
%     \label{fig:scene_simu_poster}
%     \hfill\centering\includegraphics[width=0.33\linewidth]{figure/scene/scene_simu_poster.png}
%     \label{fig:scene_simu_poster_planar_traj}
%     \hfill\centering\includegraphics[width=0.33\linewidth]{figure/scene/scene_simu_poster.png}
%     \label{fig:scene_simu_poster_6dof_traj}
% }

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subfigure[\textit{simu\_checkerboard}]
% {    
%     \hfill\centering\includegraphics[width=0.33\linewidth]{figure/scene/scene_simu_checkerboard.png}
%     \label{fig:scene_simu_checkerboard}
%     \hfill\centering\includegraphics[width=0.33\linewidth]{figure/scene/scene_simu_checkerboard.png}
%     \label{fig:scene_simu_checkerboard_planar_traj}
%     \hfill\centering\includegraphics[width=0.33\linewidth]{figure/scene/scene_simu_checkerboard.png}
%     \label{fig:scene_simu_checkerboard_6dof_traj}
% }

% \begin{figure}[t]
%     % \centering
%     \subfigure[\textit{rpg\_bin\_6DoF}]
%     {
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_rpg_bin.png}
%         \label{fig:scene_rpg_bin}
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_rpg_bin.png}
%         \label{fig:scene_rpg_bin_6DoF_traj}
%     }

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \subfigure[\textit{rpg\_box\_6DoF}]
%     {
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_rpg_box.png}
%         \label{fig:scene_rpg_box}
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_rpg_box.png}
%         \label{fig:scene_rpg_box_6DoF_traj}
%     }

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \subfigure[\textit{rpg\_desk\_6DoF}]
%     {    
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_rpg_desk.png}
%         \label{fig:scene_rpg_desk}
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_rpg_desk.png}
%         \label{fig:scene_rpg_desk_6DoF_traj}
%     }

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \subfigure[\textit{rpg\_monitor\_6DoF}]
%     {    
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_rpg_monitor.png}
%         \label{fig:scene_rpg_monitor}
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_rpg_monitor.png}
%         \label{fig:scene_rpg_monitor_6DoF_traj}
%     }    
%     \caption{xxx}
%     \label{fig:rpg_scene_trajectory}
% \end{figure}

% \begin{figure}[t]
%     % \centering
%     \subfigure[\textit{upenn\_indoor\_flying1\_6DoF}]
%     {
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_upenn_indoor_flying1.png}
%         \label{fig:scene_upenn_indoor_flying1}
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_upenn_indoor_flying1.png}
%         \label{fig:scene_upenn_indoor_flying1_6DoF_traj}
%     }

%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \subfigure[\textit{upenn\_indoor\_flying3\_6DoF}]
%     {
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_upenn_indoor_flying3.png}
%         \label{fig:scene_upenn_indoor_flying3}
%         \hfill\centering\includegraphics[width=0.48\linewidth]{figure/scene/scene_upenn_indoor_flying3.png}
%         \label{fig:scene_upenn_indoor_flying3_6DoF_traj}
%     }
%     \caption{xxx}
%     \label{fig:upenn_scene_trajectory}
% \end{figure}


